Post-Training Neural Network Pruning using Graph Curvature

This paper provides a fresh view of the neural network (NN) pruning problem through the lens of graph theory. To achieve effective pruning, we aim to identify the main NN data flows and the corresponding NN connections that are most and least important for the performance of the full model. Unlike the standard approach to NN data flow analysis, which is based on information theory, we employ the notion of graph curvature, specifically Ollivier-Ricci curvature (ORC). ORC has been successfully used to identify important graph edges in various domains such as road traffic analysis, biological networks, and social networks. In particular, edges with negative ORC are considered bottlenecks and are therefore critical to the graph's overall connectivity, whereas positive-ORC edges are less essential. We use this intuition for NNs to (1) construct a graph induced by the NN structure and introduce the notion of neural curvature (NC) based on ORC; (2) calculate curvatures based on activation patterns for a set of input examples; and (3) demonstrate that NC can be used to rank edges according to their importance for overall NN functionality. We evaluate our method through pruning experiments on a variety of small and medium size models trained on three image datasets: MNIST, CIFAR-10, and CIFAR-100. The results indicate that our method can identify a larger number of unimportant edges compared to existing pruning methods.

==> implementation.tex <==
\section{Neural Ricci Curvature Implementation}\label{sec:implementation}
The overall implementation of neural Ricci curvature is based on the \texttt{GraphRicciCurvature} library~\citep{ni2019community}, which efficiently handles graph construction and curvature computations on the CPU using Python. 
To better integrate with PyTorch and leverage GPU acceleration, which is widely used in NN training, we reimplemented parts of the library in PyTorch, enabling curvature computations directly on the GPU. Specifically, while the Wasserstein distance computation still needs to be performed on the CPU (effectively solving a linear program for each edge), the shortest-path calculation can be performed on the GPU, as follows.

Since the neural graph $G_{f_\theta}$ is directed and has a layer-by-layer structure, we can apply dynamic programming to compute the shortest-path distances required for the Wasserstein distance in the curvature calculation. %Specifically, we use a dynamic programming formulation of the min-plus matrix multiplication. 
%
For a neural graph $G_{f_\theta}$, we define an adjacency cost matrix of layer $l$ as a matrix
$C^{(l)}$, where each entry 
%\begin{equation*}
$C^{(l)}_{ij} = w_{f_\theta}\!\left(v_{i,l-1}, v_{j,l}\right)$
%\end{equation*}
is the cost associated with the edge from neuron $v_{i,l}$ to neuron $v_{j,l+1}$.

Let $D^{(k,l)}$ denote the minimum accumulated path cost between neurons in layer $t$ and neurons in layer $l$, for any $k < l$.
For $l = k+1$, we set $D^{(k,l)} = C^{(l)}$.
For $l > k+1$, the distance matrix is computed via the dynamic programming recursion
\begin{equation*}
    D^{(k,l)}_{ij} = \min_m \left( D^{(k,l)}_{im} + C^{(l)}_{mj} \right).
\end{equation*}
%This procedure performs a single forward pass through the network layers and does not rely on iterative convergence; rather, it computes shortest-path costs in a directed acyclic graph.
%
This procedure can be efficiently implemented on a GPU, thereby allowing us to scale our approach to large CNNs.
%using a fully chunked approach, which reduces memory usage and fully exploits the parallel computing capabilities of modern GPUs. 
%In our experiments, we use this method together with the \texttt{ricci} library~\citep{ni2019community} to compute Ollivier-Ricci curvature for large neural networks.

Finally, to approximate the limit of the neural curvature as Definition~\ref{def:graph_ricci}, we set $\alpha = 0.9$. 
%Based on our empirical observations, the curvature stabilizes for $\alpha \ge 0.5$, indicating that the results are largely insensitive to the specific choice of $\alpha$ within this range.
Based on our empirical observations, the $\alpha$-curvature does not change significantly beyond that point, so it is a good compromise between approximation accuracy and numerical stability.


